A comprehensive review and new taxonomy on superpixel segmentation

Superpixel segmentation consists of partitioning images into regions composed of similar and connected pixels. Its methods have been widely used in many computer vision applications since it allows for reducing the workload, removing redundant information, and preserving regions with meaningful features. Due to the rapid progress in this area, the literature fails to catch up on more recent works among the compared ones and to categorize the methods according to all existing strategies. This work fills this gap by presenting a comprehensive review with new taxonomy for superpixel segmentation, in which methods are classified according to their processing steps and processing levels of image features. We revisit the recent and popular literature according to our taxonomy and evaluate 20 strategies based on nine criteria: connectivity, compactness, delineation, control over the number of superpixels, color homogeneity, robustness, running time, stability, and visual quality. Our experiments show the trends of each approach in pixel clustering and discuss individual trade-offs. Finally, we provide a new benchmark for superpixel assessment, available at https://github.com/IMScience-PPGINF-PucMinas/superpixel-benchmark.

==> sections/experiments.tex <==
\section{Experimental setup}\label{sec:setup}

\subsection{Methods and datasets}\label{sec:methods_datasets}

In this work, we identified $14$ open source codes from the recent superpixel literature: DISF~\cite{BELEM-2020-DISF}, RSS~\cite{CHAI-2020-RSS}, ODISF~\cite{BELEM-2021-ODISF}, IBIS~\cite{BOBBIA-2021-IBIS}, DRW~\cite{KANG-2020-DRW}, DAL-HERS~\cite{PENG-2022-DAL-HERS}, ISF~\cite{VARGAS-2019-ISF}, GMMSP~\cite{BAN-2018-GMMSP}, SCALP~\cite{GIRAUD-2018-SCALP}, SNIC~\cite{ACHANTA-2017-SNIC}, SH~\cite{WEI-2018-SH}, LNSNet~\cite{ZHU-2021-LNS-Net}, SICLE~\cite{BELEM-2022-SICLE-boost}, and LSC~\cite{CHEN-2017-LSC,LI-2015-LSC}. In addition, we include the $6$ methods recommended as state-of-the-art in \cite{STUTZ-2018-BENCHMARK}: SLIC~\cite{ACHANTA-2012-SLIC}, SEEDS~\cite{BERGH-2012-SEEDS}, ERS~\cite{LIU-2011-ERS}, ETPS~\cite{YAO-2015-ETPS}, CRS~\cite{CONRAD-2013-CRS}, and ERGC~\cite{BUYSSENS-2014-ERGC}. Finally, a grid segmentation (GRID) was used as a baseline. 
Regarding implementation, we used the code of SEEDS, CRS, and ERGC available in the benchmark of Stutz et. al~\cite{STUTZ-2018-BENCHMARK}. Also, we implemented grid segmentation. For the other methods, we use the original authors' code. Furthermore, we set the parameters according to the recommended ones in their respective articles and we did not perform fine-tuning. All evaluated methods allow some control over the number of superpixels generated. In our experiments, we assess segmentations with $K \approx \{25, 50, 75, 100, 200, 300, 400, 500, 600, 700, 800, 900, 1000\}$ desired superpixels, except for the robustness evaluation, with only $K \approx 400$ superpixels.


\input{sections/experiments/datasets}

\input{sections/experiments/measures}


\section{Results}\label{sec:results}

In this Section, we evaluate $21$ superpixel methods according to different aspects. First, we evaluate connectivity, examining the number of superpixels with distinct labels regardless of their connectivity and the number of connected components (Section~\ref{sec:connectivity}). Some superpixel methods include a merging step after the segmentation to ensure connectivity. In this work, we include a merging step as post-processing on methods that do not guarantee connectivity. In Section~\ref{sec:quantitative}, we quantitatively evaluate object delineation, color homogeneity, and compactness. Also, we summarize these results with a boxplot analysis. As \cite{NEUBERT-2013-EVALUATING,STUTZ-2018-BENCHMARK}, we evaluated the methods' stability using the evaluation measures' minimum (min), maximum (max), and standard deviation (std) in Section~\ref{sec:stability}. Afterward, we assessed robustness and runtime in Sections ~\ref{sec:robustness} and ~\ref{sec:runtime}, respectively. Finally, in Section~\ref{sec:qualitative}, we perform a qualitative evaluation concerning the smoothness of the contours of superpixels, their compactness, and their adherence to the images' boundaries. The superpixel methods and codes used in this work are available in our superpixel evaluation benchmark at https://github.com/IMScience-PPGINF-PucMinas/superpixel-benchmark.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/charts/connectivity.pdf}
    \caption{Number of generated superpixels in relation to the desired number of superpixels (top row) and the number of not connected superpixels in relation to the number of generated superpixels (bottom row) on Birds, Sky, ECSSD, and Insects datasets.}
    \label{fig:connectivity}
\end{figure}




\input{sections/experiments/connectivity}

\input{sections/experiments/quantitative}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/results/charts/stability_delineation.pdf}
    \caption{Results for minimum BR, maximum UE, and standard deviation of BR and UE on Birds, Sky, ECSSD, and Insects datasets.}
    \label{fig:stability:delineation}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/results/charts/stability_homogeneity.pdf}
    \caption{Results for minimum and standard deviation of EV and SIRS on Birds, Sky, ECSSD, and Insects datasets.}
    \label{fig:stability:homogeneity}
\end{figure}



\input{sections/experiments/stability}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/results/charts/noise.pdf}
    \caption{Influence of average blur (top row) and salt and pepper noise (bottom row) for $K \approx 400$ on Birds dataset.}
    \label{fig:robustness}
\end{figure}

\input{sections/experiments/robustness}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/results/charts/time.pdf}
    \caption{Runtime in seconds on Birds, Sky, ECSSD, and Insects datasets.}
    \label{fig:time}
\end{figure}

\input{sections/experiments/runtime}


\input{sections/experiments/qualitative}





